A Survey on Data Contamination for Large Language Models

Recent advancements in Large Language Models (LLMs) have demonstrated significant progress in various areas, such as text generation and code synthesis. However, the reliability of performance evaluation has come under scrutiny due to data contamination-the unintended overlap between training and test datasets. This overlap has the potential to artificially inflate model performance, as LLMs are typically trained on extensive datasets scraped from publicly available sources. These datasets often inadvertently overlap with the benchmarks used for evaluation, leading to an overestimation of the models' true generalization capabilities. In this paper, we first examine the definition and impacts of data contamination. Secondly, we review methods for contamination-free evaluation, focusing on three strategies: data updating-based methods, data rewriting-based methods, and prevention-based methods. Specifically, we highlight dynamic benchmarks and LLM-driven evaluation methods. Finally, we categorize contamination detecting methods based on model information dependency: white-Box, gray-Box, and black-Box detection approaches. Our survey highlights the requirements for more rigorous evaluation protocols and proposes future directions for addressing data contamination challenges.

==> tables/assumption.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Authors} & \textbf{Assumption} & \textbf{Certain Tasks}\\
\hline
\textbf{DCQ} & \cite{golchin2023data} & Verbatim-Memorization  & \texttimes \\
\hline
\textbf{Guided Instruction} & \cite{golchin2023time} & Verbatim-Memorization &\texttimes\\
\hline
\textbf{DE-COP} & \cite{duarte2024decopdetectingcopyrightedcontent} & Verbatim-Memorization &\texttimes\\
\hline
\textbf{CDD} & \cite{dong-etal-2024-generalization} & Output Distribution  &\texttimes \\
\hline
\textbf{TS-Guessing} & \cite{deng2023investigating} & Verbatim-Memorization  &\texttimes \\
\hline
\textbf{ATD} & \cite{ranaldi-etal-2024-investigating} & Verbatim-Memorization & \checkmark\\
\hline
\textbf{Data Archaeology} & \cite{chang-etal-2023-speak} & Verbatim-Memorization & \checkmark\\
\hline
\end{tabular}
\caption{Black-box contamination detection methods, details of the assumptions underlying these approaches can be found in Appendix \ref{sec:assumption detail}.}
\label{tab:contamination method assumption}
\end{table*}

==> tables/detection_methods.tex <==
\begin{tabular}{|c|c|c|>{\centering\arraybackslash}m{6.5cm}|}
\hline
\multirow{1}{*}{\textbf{Method Category}} 
& \multicolumn{1}{c|}{\textbf{Method Name}}
& \multirow{1}{*}{\textbf{Authors}} & \multirow{1}{*}{\textbf{Description}} \\
\hline

& PAC & \cite{ye-etal-2024-data} & Calculates polarization distances through input perturbations to detect contamination in membership inference attacks. \\
\cline{2-4}
& MIN-K\% & \cite{shi2024detectingpretrainingdatalarge} & Detects pretraining data contamination using outlier token probabilities. \\
\cline{2-4}
\multirow{2}{*}{\textbf{Gray-Box Detection}} 
& DC-PDD & \cite{zhang2024minkimprovedbaselinedetecting} & Incorporates corpus frequency divergences to reduce false positives in contamination detection. \\
\cline{2-4}
& Perplexity-based Detection & \cite{li2023estimatingcontaminationperplexityquantifying} & Uses perplexity scores to detect memorization and contamination in models.\\
\cline{2-4}
& Adversarial Compression Ratio (ACR) & \cite{schwarzschild2024rethinkingllmmemorizationlens} & Quantifies memorization through input-output token efficiency in the model's responses. \\
\hline
\end{tabular}


==> tables/ngram.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{4cm}|>{\centering\arraybackslash}p{4cm}|>{\centering\arraybackslash}p{3cm}|}
\hline
\textbf{Model}   & \textbf{Author} & \textbf{Method} & \textbf{Token-Level} \\ 
\hline
\textbf{GPT3} & \cite{brown2020language}   & n-gram (n=13)       & \texttimes    \\ \hline
\textbf{Palm} & \cite{chowdhery2023palm}    & n-gram        & \checkmark      \\ \hline
\textbf{Llama2} & \cite{touvron2023llama2} & extended n-gram      & \checkmark     \\ \hline
\textbf{GPT4} & \cite{openai2024gpt4technicalreport}  & n-gram (n=50)    & \texttimes  \\ \hline
\textbf{Phi-4} & \cite{abdin2024phi4technicalreport}  & hybrid n-gram   & \texttimes    \\ \hline
\end{tabular}
\caption{N-gram method used for contamination detection, Token-level refers to the standard for measuring contamination scores using tokens.}
\label{tab:ngram}
\end{table*}

